Learning from Rational Behavior: Predicting Solutions to Unknown Linear Programs

We define and study the problem of predicting the solution to a linear program (LP) given only partial information about its objective and constraints. This generalizes the problem of learning to predict the purchasing behavior of a rational agent who has an unknown objective function, that has been studied under the name "Learning from Revealed Preferences". We give mistake bound learning algorithms in two settings: in the first, the objective of the LP is known to the learner but there is an arbitrary, fixed set of constraints which are unknown. Each example is defined by an additional known constraint and the goal of the learner is to predict the optimal solution of the LP given the union of the known and unknown constraints. This models the problem of predicting the behavior of a rational agent whose goals are known, but whose resources are unknown. In the second setting, the objective of the LP is unknown, and changing in a controlled way. The constraints of the LP may also change every day, but are known. An example is given by a set of constraints and partial information about the objective, and the task of the learner is again to predict the optimal solution of the partially known LP.

==> 2d_append.tex <==
\section{Finite Mistake Bound with Arbitrary Precision in 2D}\label{sec:2d}

 We restrict our attention to two dimensions, so $\bbx \in \R^2$ and $\cP = \{ \bbx \in \R^2 : A \bbx\leq \bbb\}$ is the unknown polytope where $A$ has $m>2$ rows. The nice thing about working in two dimensions is that each edge of the polytope corresponds to an unknown constraint.  Thus, if we can learn edges, then we can get the rows of $A$ and the entries of $\bbb$.   We show that the questionable region does not cause a problem in this case.  
\subsection{Algorithm}

At each round, the observer will make a prediction $\hat\bbx^{(t)}$ based on the previous solutions he has seen, and if he is wrong, he will update his guess for the unknown constraints of the LP.  Given Assumption \ref{assumpt:bind} and $d=2$, when the known constraint binds, there is exactly one constraint in the underlying LP that binds as well.  Using Lemma \ref{lem:edge}, we know that once we see three points that are collinear then all three points must bind the same constraint. Thus, we can combine these observations to learn the edge $\bbe$ where
$$
\bbe = \{\bbx\in \R^2 : A_i \bbx = b_i \text{ for some } i \in [m] \}.
$$

We will adapt our notation we used in our presentation of $\learnedge$.  We introduce the set $Z \utt$ as the collection of pairs $(\bbx^{(t')},\hat e^{(t')} )$ where $\bbx^{(t')} \in X\utt$ in not on a learned edge at round $t$ and we made a mistake by guessing point $\hat\bbx\utt \in \hat e\utt$.  We then define the set $D_e\utt$ for each $e \in E\utt$ as
$$
D_e\utt = \{\bbx \in \bar X\utt : (\bbx,e) \in Z\utt \}.
$$

Now for each $e \in E\utt$ where $B_e\utt \neq \emptyset$ and $D_e\utt \neq \emptyset$ then we define the swap set $W_e\utt$ as such
$$
W\utt_e = D_e\utt.
$$
For all other edges, we define $W\utt _e = B_e\utt$.  We then define the total swap set $W\utt$ as
$$
W\utt = \bar X\utt \cup \left\{ \bigcup_{e \in E\utt} W_e\utt\right\}
$$

Further we define the set $\bar Z_e\utt  = \{(\bbx,e) \in Z\utt : \bbx \in \bar\cN\utt \}$.  Our modified learning algorithm for the two dimensional case, which we call $\learntwo$, has the following predicton rules:
\begin{enumerate}[label=\textbf{P.\arabic*}]
\item\label{p1-2d} First, if $\bbx^*$ is recorded and $\bbx^*\in\cN\utt$, then predict $\hat\bbx\utt \gets \bbx^*$;

\item\label{p2-2d} Else if $\bar X\utt \cup B\utt \neq \emptyset$ then predict 
$$\hat\bbx\utt \gets \myargmax_{\bbx \in W\utt} \bbc\cdot \bbx.$$
%\begin{enumerate}
%	\item\label{p2a-2d} If $\bby = \myargmax_{\bbx \in \bar X\utt \cup B\utt } \bbc\cdot \bbx$ and there exists $(\bbz^*,\hat e) \in \bar Z\utt$ such that $\bby \in \hat e$ and 
%	$$\bbz^* = \myargmax_{\bbz: (\bbz,\hat e) \in \bar Z\utt}\bbc\cdot \bbz $$
%	 then $\hat \bbx\utt \gets \bbz^*$.  
%	
%	\item\label{p2b-2d} Else $\hat\bbx\utt \gets \myargmax_{\bbx \in \bar X\utt \cup B\utt } \bbc\cdot \bbx$.  
%\end{enumerate}

\item \label{p3-2d}  Else predict $\hat\bbx\utt$ as an arbitrary point outside of $E\utt$ and $X\utt$;
\end{enumerate}

ADD HIGH LEVEL OF PREDICTION RULES

Next we describe how $\learntwo$ updates this information when we make a mistake.  As we said in our presentation of the update rules in $\learnedge$, if an update rule does not mention updating a quantity, then it remains the same the next round except for the quantity $X\utt$ which we update each round by adding the optimal point each day $X\uttf \gets X\utt \cup \bbx\utt$.

\begin{enumerate}[label=\textbf{U.\arabic*}]
\item\label{u1-2d} If $\bbx\utt \notin \bar\cN\utt$ then $\bbx^* \gets \bbx\utt$.  
\item\label{u2- 2d} Else if $\bbx\utt \notin \bar X\utt$ and there is no edge in $E\utt$ such that $\bbx\utt \in e$, then we check if there exists a pair $\bbx,\bbx' \in X\utt$ such that $\{\bbx,\bbx',\bbx\utt \}$ are collinear, in which case we add a new edge $e$ to the edges: $E\uttf \gets E\utt \cup \{ e\}$;
\item\label{u2-3d}  Else if there is no $ e \in E\utt$ such that $\bbx\utt \in e$ then check if $\bbx\utt$ is collinear with two other points in $X\utt$, in which case we add this line as an edge $e$ and $E\uttf \gets E\utt \cup \{ e\}$. 
\begin{enumerate}
	\item \label{u2a-2d} If $\bbx\utt \in \bar X\utt$ then we update $Z\uttf \gets Z\utt \cup\left\{ (\bbx\utt, \hat e\utt) \right\}$ where $\hat\bbx\utt \in \hat e \utt$.
	\item \label{u2b-2d} Else $X\uttf \gets X\utt \cup \{\bbx\utt \}$.  Further, we update the corresponding quantities in  $D_e\uttf$, $W_e\uttf$ for each edge $e \in E\utt$ as well as $W\uttf$.  .  
\end{enumerate}
\end{enumerate}

 ADD HIGH LEVEL OF UPDATE RULES

\subsection{Analysis}

\begin{lemma}
Fix some $t$, for each $(\bbx,\hat e) \in Z\utt$, we know that $\bbx\in \bar X\utt$ has higher objective than any other feasible point in $\cP$ along edge $\hat e$.  
\end{lemma}
\begin{proof}
Consider the day where we added $(\bbx\utt, \hat e \utt)$ to $Z\utt$ so that both our predicted point $\hat\bbx\utt$ and observed point $\bbx\utt$ were in $\bar\cN\utt$.  The reason why we guessed $\hat\bbx\utt \in \hat e \utt$ instead of $\bbx\utt \in \bar X \utt$ was because $\bbc\cdot\bbx\utt < \bbc\cdot\hat\bbx\utt$ and so $\hat\bbx\utt$ must be infeasible.  

Because the new con
\end{proof}


We will bound the number of mistakes we ever make by showing that our update rules cover all possible mistakes and that each update rule can only occur a few number of times.  We first show that if we ever use prediction rule \ref{p2-2d} at time $t$, then we will never make a mistake where $\bbx\utt \in \bar X\utt$.  
\begin{lemma}
If we use \ref{p2-2d} to make prediction $\hat\bbx\utt$ then we cannot have $\bbx\utt \neq \hat\bbx\utt$ and $\bbx\utt \in \bar X\utt$.  
\end{lemma}
\begin{proof}
Note that in \ref{p2-2d} always picks the point in $W\utt$ with the highest objective.  The only worry is that in the swap set $W\utt$ we may pick a point with lower objective than the true optimal $\bbx\utt$.  However, $\bbx\utt \in X\utt$ so the point $\hat\bbx\utt$ must have objective no smaller than $\bbc\cdot\bbx\utt$.  
\end{proof}

\begin{lemma}
In $\learntwo$ if we ever use update rule \ref{u2a-2d}, then there exists $\hat e \utt \in E\utt$ such that $\hat\bbx\utt \in \hat e \utt$.  
\end{lemma}
\begin{proof}
Because $\bbx\utt \in \bar X\utt$, we know that $\bar X\utt$ is nonempty and thus we would have used \ref{p2-2d} to make our prediction.  We would guess the point in $W\utt$ with highest objective.  If we were to use \ref{p2-2d} then we know our guess would be on an edge $\hat e\utt \in E\utt$ with $\hat\bbx\utt \in \hat e\utt$, because we must have guessed a point with no smaller objective value than the actual solution, which by uniqueness of our solution must be infeasible but all points in $\hat X\utt$ are feasible that day.  

If we use \ref{p2-2d}, then we know from the previous lemma that if we make a mistake at day $t$ then $\bbx\utt \notin \bar X\utt$, hence we would not have used \ref{u2a-2d} to make an update.   
\end{proof}





We first show that we always use an update rule when we make a mistake.
\begin{lemma}
Each time $\learntwo$ makes a mistake in the Known Objective Problem when $d=2$, we use one update rule given above in \ref{u1-2d} and \ref{u2-2d}.  
\end{lemma}
\begin{proof}
Specifically, what we need to show is that there is never the time we make a mistake and there is some edge $e \in E\utt$ such that $\bbx\utt \in e$.  
\end{proof}


As we showed in our analysis of $\learnedge$ in Lemma \ref{}, we know the number of updates we need to do in $\learntwo$ 


We then consider mistakes of the type when the additional constraint binds each day.  Note that we are no longer updating some edge set $E$, but rather we are creating a feasible region by learning the actual constraints of the underlying LP in \eqref{eq:LP}.  

\begin{lemma}
We assume that Assumptions \ref{assumpt:rank} and \ref{assumpt:bind} hold.  For each round $t$, every row of $A\utt$ and $\bbb\utt$ in $\learntwo$ is a row of the unknown matrix $A$ and the unknown right hand side vector $\bbb$, respectively.
\label{lem:2d-constraints}
\end{lemma}
\begin{proof}
$\uptwo$ adds a row to $A\utt$ and $\bbb\utt$ after observing three collinear points that bind the added constraint on the days they were seen.  By Lemma \ref{lem:edge}, we know that these three points form an edge of the underlying polytope, so for $d=2$ only one row of the underlying matrix binds.  Thus, we learn $\bbe^i = \{\bbx \in \R^2: A_i\bbx = b_i \}$ for some $i \in [m]$ after seeing three collinear points.  
\end{proof}

Note that in $\predtwo$, once we have learned a constraint, there is the case when we may not know the direction of the inequality because we have only seen points that bind that constraint.  This can only occur when we only know a single constraint of the underlying LP and we have never seen a point that does not bind that constraint.  In that case, $\predtwo$ will only guess points that bind the added constraint and the learned constraint.  If we ever guess incorrectly, then the adversary must have shown a point that does not bind the constraint we have learned.  Further, once we know the direction of the inequality in the constraints, then we use \eqref{eq:predtwo} to find the best feasible point that we know so far.  Hence, every time we make a mistake, the adversary is showing a point that binds a constraint that is not learned yet.  

Let us consider mistakes of the following type
\begin{equation}
M^{2D}_1 = \sum_t \1\left\{\hat\bbx\utt \neq \bbx\utt : \bp\utt\cdot\bbx\utt = q\utt \right\}
\label{eq:mistake1_2d}
\end{equation}

We then have the following result.

\begin{lemma}
We assume that Assumptions \ref{assumpt:rank}, \ref{assumpt:bind}, and \ref{assumpt:distinct} hold.   If an observer uses $\learntwo(\cA)$ against $\cA$ then we have 
$$
M^{2D}_1 \leq 3m
$$
$\quad$ where $M^{2D}_1$ is given in \eqref{eq:mistake1_2d}
\label{lem:2d-m1}
\end{lemma}
\begin{proof}
We only consider the case that the added constraint each day binds.   It must then be the case that $\bbx\utt$ binds one of the rows of $A$ and  $\bbb$.  From Lemma \ref{lem:2d-constraints}, we know that each time we update via \eqref{eq:predtwo} then we only make a mistake if the point we predict violates an unknown constraint and the actual solution binds a constraint we have not learned.  Further, if we do not use \eqref{eq:predtwo} to predict $\hat\bbx\utt$, then we can only make a mistake if again we see a point that binds a constraint we have yet to learn.  

Thus, the only way we can make a mistake when the added constraint does not bind is if the actual point is binds a constraint that has not been learned yet.  By Assumption \ref{assumpt:distinct} and because we learn constraints after seeing three points that are collinear by Lemma \ref{lem:edge}, the lemma follows.  

By Assumption~\ref{assumpt:distinct}, each time $\bbx\utt$ is on an unknown constraint then it must be distinct from other points on that edge.  This can occur at most $3m$ times because there are $m$ rows of $A$ and we learn the rows after seeing three distinct points that bind the unknown constraint. 
\end{proof}

Putting all the pieces together, we bound the number of mistakes of $\predtwo$ in Theorem~\ref{thm:mistake_2d}. 
\begin{theorem}
If Assumptions~\ref{assumpt:rank} and \ref{assumpt:distinct} hold, the procedure that has the observer make predictions based on $\predtwo$ and updates by $\uptwo$ can make a finite number of mistakes $M$, where
$$
M =O(m).
$$
\label{thm:mistake_2d}
\end{theorem}
\begin{proof}
The proof is immediate from Lemmas~\ref{lem:mistake1}~and~\ref{lem:2d-m1}.
\end{proof}


==> Proofs/corner.tex <==
\ifnum\final=0
\begin{proof}
\else
\begin{proof}[Proof of Lemma~\ref{lem:corner-case}]
\fi
%% Recall that edges are defined as the intersection of $d-1$ hyperplanes
%% in $\cP$, thus every point on $e$ must bind at least $d-1$ constraints
%% of $A\bbx\leq \bbb$.  Since $e \subseteq \tN\utt$, we would have $d$
%% constraints bind in the polytope $\cP\utt = \cP\cap \cN\utt$ along all
%% points of $e$.  By
%% Assumptions~\ref{assumpt:vertex}~and~\ref{assumpt:bind}, the observed
%% solution $\bbx\utt$ needs to bind exactly $d$ constraints and be a
%% vertex.  There can be no vertices along this edge $e$ due to
%% Assumption \ref{assumpt:bind}. Hence, $\bbx^\cN$ cannot be on this
%% edge.\snote{rewrote the proof}

Note that the observed solution $\bbx\utt$ is a vertex in the polytope
$\cP\utt = \cP\cap\tN\utt$, that is an intersection of \emph{exactly}
$d$ constraints by Assumption~\ref{assumpt:bind} and
Assumption~\ref{assumpt:vertex}. Note that all points in $e$ binds at
least $d - 1$ constraints in $\cP$ and since $e\subseteq \tN\utt$,
then all points in $e$ binds at least $d$ constraints in $\cP\utt$.
It follows that any vertex of $\cP\utt$ on $e$ must bind at least
$(d+1)$ constraints, which rules out the possibility of $\bbx\utt$
being on $e$.
\end{proof}


==> Proofs/lem_stoch_case.tex <==
%Let $E$ denote the set of edges of $P$, and
%\ar{Changed this proof substantially}\sj{thanks!}
First, since all of the points $x_1,\ldots,x_t$ are drawn i.i.d. from $\cD$, we observe by symmetry that the event we are interested in is distributed identically to the following event: That when we draw a set of $t$ points $X'=\{x_1,\ldots, x_{t}\}$ i.i.d. from $\cD$ and select an index $i \in \{1,\ldots,t\}$ uniformly at random, $x_i \not\in \mathrm{conv}(X' \setminus \{x_i\})$. In other words
 $$\Pr_{x_1,\ldots,x_t \sim \cD}[x_t\not\in \mathrm{conv}(X)] = \Pr_{x_1,\ldots,x_t \sim \cD, i \sim \{1,\ldots,t\}}[x_i\not\in \mathrm{conv}(X' \setminus \{x_i\})].$$
We analyze the quantity on the right hand side instead, fixing the choices of $x_1,\ldots,x_t$, and analyzing the probability only over the randomness of the choice of index $i$.
For each edge $e\in E_{\cP}$, let $X_e' = X' \cap e$.  %be the set of points on $e$ which are in $X'$. 
Since each edge lies on a one dimensional subspace, there are at most two extreme points in $x^e_1,x^e_2 \in X_e'$
that lie outside of the convex hull of other points -- i.e. such that $x^e_1 \not\in \mathrm{conv}(X'\setminus\{x^e_1\})$ and $x^e_2 \not\in \mathrm{conv}(X'\setminus\{x^e_2\})$.
%% A point is an extreme point among a set of points if it is not in
%% the convex hull of other points, and there are at most two extreme
%% points
We note that when we choose an index $i$ uniformly at random, the probability that we select a point $x \in X'_e$ is exactly $|X'_e|/t$, and conditioned on selecting a point $x \in X'_e$, the probability that $x$ is an extreme point (i.e.  $x \in \{x^e_1,x^e_2\}$) is at most $2/|X'_e|$.
Hence, we can calculate
\begin{align*}
\Pr\left[ x_i \not \in \mathrm{conv}(X'\setminus \{x_i\}) \right] &=
\sum_{e\in E_{\cP}} \Pr[x_i \in X'_e] \cdot \Pr[ x_i \notin
  \mathrm{conv}(X_e'\setminus \{x_i\}) \mid x_i \in X'_e]\\
&\leq \sum_{e\in E_{\cP}} \frac{|X_e'|}{t} \cdot \frac{2}{|X_e'|} = \sum_{e\in E_{\cP}} \frac{2}{t} = \frac{2|E_{\cP}|}{t}.
\end{align*} 

==> Proofs/thm_mistakebdd.tex <==
First, we show that $\learnhull$ makes a mistake only if the true
optimal point $\bbx^{(t)}$ lies outside of the convex hull
$\cC^{(t-1)}$ formed by the previous observed optimal points $\{\bbx^{(1)}, \ldots, \bbx^{(t-1)}\}$. Suppose that at
round $t$, the algorithm predicts the point $\hat \bbx^{(t)}$ instead
of the optimal point $\bbx^{(t)}$. Since each point in $\cC^{(t-1)}$
is feasible and $\hat \bbx^{(t)}$ is the point with the highest
objective value among the points in
$\{\bbx \in \cC^{(t-1)} \mid \mathbf{p}' \cdot \bbx\leq b'\}$, then it
must be that $\bbx^{(t)}\not\in \cC^{(t-1)}$ because otherwise $\bbc\cdot\bbx^{(t)} > \bbc\cdot\hat\bbx^{(t)}$. By
Lemma~\ref{lem:stoch_case}, we also know that the probability that
$\bbx^{(t)}$ lies outside of $\cC^{(t-1)}$ is no more than $2|E_{\cP}|/t$ in expectation,
which also upper bounds the probability of $\learnhull$ making a
mistake at round $t$. Therefore, the expected number of mistakes made
by $\learnhull$ over $T$ rounds is bounded by the sum of probabilities of making a mistake in each round which is $\sum_{t=1}^T 2|E_{\cP}|/t <
2|E_{\cP}|(\ln(T) + 1)$.


==> Proofs/thm_stoch.tex <==
The procedure runs $\lceil 18\log(1/\delta)\rceil$ independent instances of the $\learnhull$ each using independently drawn examples. The independent instances are aggregated into a single prediction rule by predicting using the \emph{modal} \rynote{modal?} prediction (if one exists), and otherwise predicting arbitrarily. Hence, the aggregate prediction is correct whenever at least half of the instances of $\learnhull$ are correct.

We show that if each instance of the $\learnhull$ is run for $t = 8|E_{\cP}|$ rounds, then the probability that more than half of the instances of $\learnhull$ make a mistake on a newly drawn constraint at round $T+1$ is at most $\delta$. The result is that with probability at least $1-\delta$
the majority of instances of $\learnhull$ predict the correct optimal point, and hence the aggregate prediction is also correct.

Let $Z_i$ be the random variable that denotes the probability that the $i$th instance of the $\learnhull$ algorithm makes a mistake on a fresh example, after it has been trained \rynote{Trained?  Is this formal?}
for $8|E_{\cP}|$ rounds.
By Theorem~\ref{thm:mistakebdd}, we know $E[Z_i]\leq 1/4$ for all $i$.
%$$Z = \frac{1}{|X\utt|} \cdot \sum_{x \in X\utt} \1\{ \bbx \not \in \text{conv}(X\utt \backslash \bbx) \}.$$
Now by Markov's inequality,
% and using the result of Lemma \ref{lem:stoch_case} we have
$$
\Pr\left[Z_i \geq \frac{3}{4}\right] = \Pr\Big[Z_i \geq 3\cdot E[Z_i]\Big] \leq 1/3,
$$
for all $i$. Hence, the \emph{expected} number of instances that make a mistake is at most $1/3$. Finally, since each instance is trained on independent examples, a Chernoff bound implies that the probability that at least half of the instances of $\learnhull$ make a mistake is bounded by $\delta$.

%\ar{Do we need to invoke some mysterious theorem here? Doesn't this just follow from a Chernoff bound?}\sj{reworked}
%We then run $T= \log(1/\delta)$ independent trials of $\learnhull$ simultaneously each with $t$ fresh draws from the distribution $\cD$. We denote each trial $i$ with its own proportion $Z_i$ for its sample of points $X\utt_i$.  We use a Chernoff bound to then bound the number of trials where $Z_i \geq 2\beta$ to get
%$$
%\Prob{}{\frac{1}{T} |\{i \in [T] : Z_i \geq 2\beta \} |\geq 1/2+\epsilon} .
%$$
%Then the probability that in at least in half of the copies of the $\learnhull$, the predicted optimal point is incorrect is new optimal point is outside
%of the convex hull of at least half of the trials of $\learnhull$ is simply bounded by $(1/2)^{(\log(1/\delta))}=\delta$ by independence.
%% because the trials of $\learnhull$ use independent samples.
%
%In Theorem~\ref{thm:mistakebdd}, we showed that the $\learnhull$ only makes a mistake if the optimal point is outside of its convex hull.
%So with probability at least $1-\delta$, at least half of the trials of the $\learnhull$ predict the optimal point correctly.

%Finally, the sample complexity
%of running $6\log(1/\delta)/\beta$ trials of the $\learnhull$ is $\lceil 12|E|/\beta^2\cdot\log\left(1/\delta\right)\rceil$ as in the statement of the theorem.  Our procedure then is to run $T$ independent trials of $\learnhull$ where each trial uses $t$ samples.  

==> Proofs/thm_unknown_obj.tex <==
\ifnum\final=0
\begin{proof}
\else
We first state that the number of updates that the ellipsoid algorithm needs to make before it finds a point in $\cF$ can be bounded by the following theorem from~\cite{GLS93} which we state for completeness.
\begin{theorem}[\cite{GLS93}]
Let $\cF \subset \R^d$ be a polytope given as the intersection of linear constraints, each of which have finite bit precision $N$.  Suppose for each point $\bbv \notin \cF$, a hyperplane with finite bit precision $N$ is given that separates $\bbv$ from $\cF$.  Then the ellipsoid algorithm outputs a point $\bbv \in \cF$ or outputs that $\cP$ is empty in time $\poly(d, N)$.
\label{thm:ell_bits}
\end{theorem}

\begin{proof}[Proof of Theorem~\ref{thm:unknwon-obj}]
\fi
Note that whenever our learning algorithm makes a mistake, we can exhibit a separating hyperplane (given in \eqref{eq:sep_hyp} ), and cause the Ellipsoid algorithm to run for another iteration.  Once we have found a point $W \in \cF$ then predicting via \eqref{eq:obj_guess} will ensure we never make a mistake again.  Hence, the number of mistakes our learning algorithm can commit against an adversary is bounded by the maximum number of iterations for which the Ellipsoid algorithm can be made to run, in the worst case. 

We assume that the observer solution $\bbx\utt$ each day is on a vertex of the polytope $\cP\utt$ which is guaranteed to have coordinates specified with at most $N$ bits of precision (i.e. which can be written as integer multiples of  $1/2^N$).   Theorem \ref{thm:lin_solve} guarantees that the solution $\hat\bbx\utt$ our learning algorithm produces in \eqref{eq:obj_guess} is a vertex solution of $\cP\utt$, so $\hat\bbx\utt$
can also be written with $N$ bits of precision, by Assumption~\ref{assumpt:precision2}.  Thus every constraint in $\cF$ and hence each separating hyperplane can be written with $d\cdot  N$ bits of precision.  By Assumption \ref{assumpt:obj_precision} and Theorem \ref{thm:ell_bits}, we know that the Ellipsoid algorithm will find a point in the feasible region $\cF$ after at most $\poly(n,d,N)$ many iterations, which yields our mistake bound.

%We note that the our linear solver from Lemma \ref{lem:lin_solve} also runs in polynomial time.  This is because each round, the $\ellip$ procedure will output $\hat\bbc\utt$, which will have finite precision at most $N$ when $\bbx\utt$ and $\hat\bbx\utt$ have precision $N$ (See Section 3.2 in \cite{GLS93}).  Further, we know that $\cP\utt$ can be written with at most $m$ constraints where each constraint can be written with at most $\poly(d,N)$ bits when we assume that its vertices have precision $N$ (see Lemma 6.2.4 in \cite{GLS93}).  Hence, we can output $\hat\bbx\utt$, which is a vertex solution for the problem in \eqref{eq:obj_guess} in time $\poly(d,n,m,N)$.

%
%It remains to show that this input can be written with finite precision, which we will show inductively.  We initialize $\hat\bbc^{(1)}$ as having finite bit precision $N$ (it is just the vector of all ones).  Further from \cite{GLS93} (Lemma 6.2.4, Page 176),
%\sj{I put a citation to the book reference. Please check, as I don't have the book.}
%we know that assuming finite precision of $N$ on the vertices of $\cP\utt$ ensures that each constraint of $\cP\utt$ can be written with $\poly(d,m,N)$ bits
%%\footnote{See Lemma 6.2.4 in \cite{GLS93}}
%where $m$ is the maximum number of constraints in the polytope any day.  Hence, in time $\poly(d,m,N)$ we can find the vertex solution $\bbx^{(1)}$ which can be written with $N$ bits, by assumption.
%
%\sj{why do we need an inductive argument? can't we say the output of ellipsoid in each round has final precision?}
%\rynote{I guess we do not need it if Lemma \ref{lem:lin_solve} guarantees a vertex solution despite $\hat\bbc\utt$ maybe being arbitrary precision (I know it is not, but I think that takes an argument, hence the induction).  Modified the proof.}
%We then assume the induction hypothesis that $\bbx\utt$ and $\hat\bbx\utt$ can be written with $N$ bits of precision.  The separating hyperplane $\cH\utt$ given in \eqref{eq:sep_hyp} then has precision $N$, because it is defined by $\bbx\utt$ and $\hat\bbx\utt$.  The updated prediction $\hat\bbc\uttf$ output by $\ellip$ with that day's separating hyperplane and ellipsoid $\cE\utt$ can be written with $N$ bits of precision, as is guaranteed with the Ellipsoid Algorithm.  Once again, we use the LP solver of Lemma \ref{lem:lin_solve} to ensure that in time $\poly(d,m,N)$ we output a vertex solution $\hat\bbx\uttf$, which is assumed to have finite precision $N$.
%
%The number of mistakes we make is bounded by the number of times before we see a point in $\cF$ given in \eqref{eq:obj_feasible} where each separating hyperplane can be written with finite precision $N$.  Hence we have $T_{EA} = \poly(n,d,N)$ many mistakes.
\end{proof}

==> colinear.tex <==
\section{Subroutines for $\learnedge$}
\label{sec:sub}
We first describe a procedure to detect collinear points. The Procedure $\coline$ in Algorithm~\ref{alg:coline} takes a set of points $X$
and a new point $\bbz$ as inputs and checks whether $\bbz$ and any two points in $X$ form a line. If so, the procedure returns that line. Otherwise, it returns the empty set.
It is easy to see that the running time of $\coline(X,\bbz)$ is $O(d |X|^2)$.  We simply check if there is any pair $\bbx,\bby \in X$ such that $(\bbz - \bby) = \lambda \cdot (\bbx - \bbz)$ for $\lambda \in \R$, in which case we output the line that $\bbx,\bby,$ and $\bbz$ is on.
\begin{algorithm}[!]
\SetAlgoNoLine{
 \begin{algorithmic}
 \Procedure{$\coline$}{$X, \bbz$}\SetAlgoNoEnd
 \State $e\gets\emptyset$ and $\lambda = \bot$ .
 \hspace{93mm} $\triangleright$ Initialize
 \State\For{$\bbx,\bby \in X$}{
 	Set $\bbw^1 = (\bbx - \bby)$ and $\bbw^2 = (\bbx - \bbz)$
	 \State\For{$j \in [d]$}{
	 
\If{$w_j^1 = 0$ and $w_j^2 \neq 0$ or $w_j^1 \neq 0$ and $w_j^2 = 0$}{
	EXIT LOOP;
}	\uElseIf{$\lambda == \bot$}{
		\State Set $\lambda \gets w_j^1/w_j^2. $
	}
	\uElseIf{$\lambda \neq w_j^1/w_j^2$}{
		EXIT LOOP;
	}
\Else{
	\State $e \gets \{(\bbx- \bbz)\cdot t+ \bbz : t \in \R \}$.
	}

}
}

\ifnum\colt=0
		\EndIf

	 \EndFor 

 \EndFor
\fi

 \Return $e$. \hspace{106mm} $\triangleright$ Output
\EndProcedure
\end{algorithmic}
}
\caption{$\coline$}
\label{alg:coline}
\end{algorithm}

Next, we describe a subroutine that identifies a vertex of the
underlying polytope $\cP$ given a questionable interval $Q_e^i$ of
length less than $1/2^{N}$. The procedure will then update the feasible
and infeasible region on that edge-space $e$. In the following, let $Z$
denote the set of points with coordinates being multiples of $1/2^N$.

\begin{algorithm}[!]
 \begin{algorithmic}
 \Procedure{$\elim$}{$(Q_e^i)\utt, F_e\utt, (Y_e^i)\utt$} 
 \State Let $a$, $b$ be the endpoints of $(Q_e^i)\utt$ where $a$ is closer
 to $F_e\utt$ and $b$ is closer to $(Y_e^i)\utt$.
 \State Let $v$ be the point in $(Q_e^i)\utt\cup\{a, b\}$ such that $v\in Z$.

 \State Let $(Q_e^i)^{(t+1)} \gets \emptyset$, $F_e^{(t+1)} \gets
 \mathrm{conv}(F_e\utt\cup \{v\})$ and $(Y_e^i)^{t+1} \gets
 \mathrm{conv}((Y_e^i)\utt\cup \{v\}).$% \Comment{Update}
\EndProcedure
\end{algorithmic}
\caption{$\elim$}
\label{alg:coline}
\end{algorithm}

\begin{lemma}
Let $Q_e^i$ be a questionable interval of length less than $1/2^N$,
and let $a$ and $b$ be the two endpoints of the interval. Then
$Q_e^i\cup \{a,b\}$ contains exactly one point $v$ in $Z$, and $v$ is a
vertex of $\cP$.
\label{lem:elim}
\end{lemma}

\begin{proof}
Note that $Q_e^i\cup \{a,b\}$ must contains a vertex in $\cP$, because
there exists a vertex that separates the disjoint intervals $F_e$ and
$Y_e^i$, and all points between these intervals are exactly the points
in $Q_e^i\cup \{a,b\}$.

Note that the length of the interval $Q_e^i$ is less than $1/2^N$, so
it contains at most one point in the finite precision set $Z$. So this point
must be $v$.
\end{proof}

Hence $\elim$ correctly eliminates the
questionable interval and updates %the corresponding 
$F_e$ and $Y_e^i$.



\iffalse
\begin{theorem}
		Consider the polytope $\cP = \{ \bbx \in \R^d : A\bbx \leq \bbb\}$ and let $\partial \cP$ denote its boundary.  If we have three point $\bbx, \bby, \bbz$ that are each collinear in $\R^d$ and 	each are on $\partial \cP$, then the minimal line segment $L$ that contains these three points must be contained in the $\partial \cP$.
		\label{thm:todo}
\end{theorem}
		This proof will follow from several claims:
		\begin{claim}
		If $\bbx$ and $\bby$ are in the interior of $\cP$ then every convex combination of these two points is also in the interior of $\cP$. 
		\end{claim}
		\begin{proof}
			We know that $A\bbx < \bbb$ and $A\bby < \bbb$, by definition of interior of $\cP$.  Hence, if we take a convex combination for $\lambda \in [0,1]$ we have 
			$$
			A\left(\lambda \bbx + (1-\lambda) \bby \right)  < \bbb. 
			$$
		\end{proof}
		\begin{claim}
		\label{clm:boundary}
		For any interior point $\bbx$ of $\cP$, any line $L$ that goes through $\bbx$ must intersect the boundary of $\cP$ (denoted by $\partial \cP$) in exactly two places.
		\end{claim}
		\begin{proof}
		We know that $L$ is convex, thus $L \cap \cP$ is also convex and a line segment.  Thus, there can be no gaps in $L \cap \cP$.  We know that if we move an arbitrary distance from the boundary point $\bbx$ along $L$ we will be at an interior point $\hat\bbx$.  Similarly we can obtain the interior point $\hat\bby$.  We know that all convex combinations of $\hat\bbx$ and $\hat \bby$ are in the interior of $\cP$ by the previous claim.  Thus, we have $|L \cap \partial\cP| = 2$.  
		\label{claim:boundary}
		\end{proof}
	We are now ready to prove Theorem~\ref{thm:todo}.
	\begin{proof}[Proof of Theorem \ref{thm:todo}]
		Let $\bbx, \bby,\bbz$ be collinear and on $\partial \cP$.  We know that the line $L$ that goes through these three points cannot go through an interior point of $\cP$, otherwise this would violate Claim~\ref{clm:boundary}. We have $L \cap \cP  = L \cap \partial \cP$ which must be convex and further a line segment that contains the points $\bbx, \bby,\bbz$.  Let $L'$ be the minimal line segment that contains the three points $\bbx,\bby,\bbz$.  So we have 
		$$
		L' \subset L \cap \partial \cP \subset \partial\cP.
		$$
	\end{proof}
%% \fi


\begin{lemma}
  Let $\bbx, \bby,\bbz$ be three distinct collinear points in the polytope
  $\cP$ such that each are on an edge of $\cP$. Then all three points are on the same edge of $\cP$.
  \label{lem:collinear}
\end{lemma}
\begin{proof}
  Without loss of generality, let us assume $\bby$ can be written as convex combination of
  $\bbx$ and $\bbz$ i.e. $\bby = \alpha \bbx + (1 -
  \alpha)\bbz$ for some $\alpha\in (0,1)$. Let $B_y = \{j \mid A_j
  \bby = \bbb_j\}$ be the set of binding constraints for $\bby$, and
  we know that $|B_y| \geq d- 1$. For any $j$ in $B_y$, we consider
  the following two cases.
  \begin{enumerate}
  \item
  At least one of $\bbx$ and $\bbz$ belongs to the hyperplane
  $\{ \bbw : A_j \bbw \leq \bbb_j\}$. Then we claim that all three points bind the same
  constraint. Assume that $A_j\bbx = \bbb_j$, then we must have
  \[
  A_j\bbz = \frac{A_j (\bby - \alpha\bbx)}{(1 - \alpha) } =
  \frac{\bbb_j - \alpha \bbb_j}{(1 - \alpha)} = \bbb_j.
  \]
  Similarly, if we assume $A_j\bbz = \bbb_j$, we will also have
  $A_j\bbx = \bbb_j$.
  \item
  None of  $\bbx$ and $\bbz$ belongs to the hyperplane
  $\{ \bbw : A_j \bbw \leq \bbb_j\}$ i.e. $A_j \bbx < \bbb_j$ and $A_j \bbz < \bbb_j$
  both hold. Then we can write
  \[
 \bbb_j =   A_j\bby = \alpha A_j \bbx + (1 - \alpha) A_j \bbz < \alpha \bbb_j + (1 - \alpha) \bbb_j = \bbb_j,
  \]
  which is a contradiction. 
\end{enumerate}
  It follows that for any $j\in B_y$, we have $A_j\bbx = A_j\bby =
  A_j\bbz = \bbb_j$. Since $|B_y| \geq d - 1$, by
  Assumption~\ref{assumpt:rank}, we know these constraints form an
  edge of the polytope, and therefore all three points must lie on the
  same edge of the polytope.
  %% By Assumption~\ref{assumpt:rank}, each of $\bbx, \bby$ and $\bbz$
  %% binds at least $(d - 1)$ constraints in $A \bbx\leq \bbb$. Then
  %% there exists three sets of rows $B_x, B_y, B_z\subset [m]$ of $A
  %% \bbx\leq \bbb$ that define the edges containing the three points
  %% respectively, and satisfy $|B_x| = |B_y| = |B_z| = d - 1$.
\end{proof}
\fi


==> conclusion.tex <==
\section{Conclusion and Open Problems}

We have considered several different problems in this paper, all relating to an observer not knowing either the objective, constraints, or both, and each day is given some information about the unknown entity that will influence the optimal solution each day.  However, we have left open several problems in the areas we have considered which we outline a few in Table \ref{table:open}.

\begin{table}[h]
\begin{center}
  \begin{tabular}{| c | c || c | c | c | }
    \cline{1-2}
    \multicolumn{2}{ |c || }{$K = $ Known, $U = $ Unknown}  \\  \hline
    Objective & Feasible Region & Dimension & Constraints &  Number of Added Constraints Each Day\\ \hline
    K & U & $d $ & $m > d+ k$ & $k>1$ \\ \hline
    U & U & $d$ & $m > d+k$ & $k \geq 0$ \\ \hline
  \end{tabular}
\end{center}
  \caption{A few open problems from our setting.}
  \label{table:open}
\end{table}

==> ellip_alg.tex <==
\section{Ellipsoid Algorithm}
The Ellipsoid Algorithm from \cite{Shor}, is a way to find a point in a convex region $\cP$ in a $d$ dimensional space by choosing smaller and smaller ellipses that always contain $\cP$, or it will output that $\cP$ is empty.  For the purposes of this paper, we need to only know that the Ellipsoid Algorithm works in the following way:
\begin{enumerate}
\item Initialize an ellipse $\cE^{(0)} \in \R^d$ such that $\cP \subset \cE^{(0)}$, set $t \gets 0$.
\item If the center point of $\cE\utt$ is not in $\cP$, then use a \emph{Separation Oracle} to find a separating hyperplane $\cH\utt$ between the center of $\cE\utt$ and where the feasible region $\cP$ resides.  Then update the ellipsoid $\cE\uttf$ to be the smallest ellipsoid to contain $\cH\utt$ and $\cE\utt$ and write $c\utt$ as the center point of this new ellipsoid.  We write this step as $(\cE\uttf, c\uttf) \gets\ellip(\cH\utt,\cE\utt)$.  
\item Else, output the center point of $\cE$.
\item If the volume of our ellipsoid ever falls below some threshold, output the $\cP$ is empty.  
\item Set $t \gets t+1$ and return to Step 2.   
\end{enumerate}

\sj{put this is algorithm format.}
We leave the \emph{Separation Oracle} in Step 2 as a black box which we make precise in the main body of our paper.  
\ifnum\final=1
\section{Formal Description of $\learnell$}
\begin{algorithm}[h]
 \begin{algorithmic}
 \Procedure{$\learnell$}{$\cA$} \Comment{Against adversary $\cA$}
 \State (\emph{Initialize})
	\State $\qquad \cI^{(0)} \gets \left(\cE^{(0)} = \{\bbz \in \R^{n\times d} : ||\bbz||_F\leq 2\}, \hat\bbc^{(0)} = \mathbf{1} \right)$
 \State (\emph{Predict})
 	\State $\qquad $ Set $\hat\bbx\utt$ as in \eqref{eq:obj_guess}.
 \State (\emph{Update})
$\qquad$ \If{$\bbx\utt \neq \hat\bbx\utt$} set $\cH\utt$ as in \eqref{eq:sep_hyp}
	\State $(\cE\utt,\hat\bbc\utt) \gets \ellip(\cH\uttb,\cE\uttb)$
	\State $\cI\utt \gets (\cE\utt,\hat\bbc\utt)$
\Else
	\State $\cI\utt \gets \cI\uttb$
\EndIf
\EndProcedure
\end{algorithmic}
\caption{Learning with Known Constraints ($\learnell$)}
\label{alg:learnellip}
\end{algorithm}
\fi


==> impossible.tex <==
\ifnum\final=0
\subsubsection{Impossibility Result} \label{sec:imp}
\else
\subsection{Impossibility Result} \label{sec:imp}
\fi


The obvious question now is if we can generalize our result in two dimensions to now hold for $m>d>2$.  We show that this is not the case, and in fact we construct a lower bound example where $m=4$ and $d=3$ where any observer can make an unbounded number of mistakes against any adversary, even against an adversary that satisfies Assumptions~\ref{assumpt:rank}--\ref{assumpt:distinct}.
% and if the objective function satisfies Assumption \ref{assumpt:obj}.}

\begin{theorem}
\label{thm:impossibility}
There exists a LP 
%that satisfies Assumption \ref{assumpt:obj} 
with 4 unknown constraints in 3 dimensions such that an adversary that satisfies Assumptions~\ref{assumpt:rank}--\ref{assumpt:distinct} can make any observer suffer an unbounded number of mistakes.
\end{theorem}
\begin{proof}[Proof Sketch]
We defer the formal proof to the appendix and only give a sketch here.  Consider an observer that learns two edges of the unknown polytope which has known objective $\bbc = (0,0,1)$.  If the observer were to ever guess points that did not reside on either edge or did not bind the added constraint each day, then the adversary could easily cause a mistake.  We then consider an observer that only guesses points that bind the added constraint and live on either learned edge.  

The main complication to the observer is that he is not sure where either of the two edges becomes infeasible.  This was easily remedied in the case when $m=d$ because we knew the edges had to intersect or are feasible everywhere.  However, in this case, we have two edges that do not intersect but are not feasible everywhere, see Figure \ref{fig:3d}.  The problem is that the observer cannot learn any constraint that intersects a learned edge because the hyperplanes the adversary chooses only gives points on either edge.  

Hence, no matter which edge the observer chooses to predict his point from, the adversary can always return the other point on the other edge as the optimal point.  After $T$ interactions, the adversary will be able to return a simple polytope which is consistent with all the observed optimal points so far. This means that the learner will make at least $T$ mistakes.  We show in the proof (in the appendix) that $T$ can be arbitrary large. 
\end{proof}

\begin{figure}[h]
\centerline{\includegraphics[width=0.3\textwidth]{3D}}
\caption{After an observer has learned two edges (shown in bold) of an unknown polytope, an adversary can have the observer make any number of mistakes by slightly perturbing the figure shown, which requires $m=4$ constraints.}
\label{fig:3d}
\end{figure}

\begin{corollary}
\label{cor-imp}
For $d\ge 3$, there exists a LP with $d+1$ unknown constraints in $d$ dimensions such that an adversary 
that satisfies Assumptions~\ref{assumpt:rank}--\ref{assumpt:distinct}
can make any
learner suffer an unbounded number of mistakes.
\end{corollary}
\ifnum\final=0
\begin{proof}
We modify the proof of Theorem~\ref{thm:impossibility} by adding dummy variables for the case that $d>3$. These dummy variables are denoted by $x_{4:d}$.
Furthermore, we add dummy  constraints $x_i\ge 0$ for all the dummy variables. 
We modify the objective of Theorem~\ref{thm:impossibility} to be $\bbc = (0, 0, 1, -1, \ldots, -1)$. This will cause all the newly added
variables to have no effect on the optimization (they should be set to $0$ in the optimal solution) and, hence, the result from Theorem~\ref{thm:impossibility}
extends to the case when $d\ge 3$.
\end{proof}
\fi

==> missing_proof5.tex <==
\section{Missing . from Section~\ref{sec:known_constr}}

\input{./thm_unknown_obj}

==> two-d.tex <==

\ifnum\final=0
\subsubsection{Two Dimensions}\label{sec:2d}
\else
\subsection{Two Dimensions}\label{sec:2d}
\fi

We start by limiting attention to two dimensions, so $\bbx \in \R^2$ and $A \in \R^{m\times 2}$ where $m>2$. Like the previous section, we will design an algorithm that allows the observer to learn edges of the polytope defined by the constraints in the LP given in \eqref{eq:LP}.  The nice thing about working in two dimensions is that each edge of the polytope corresponds to an unknown constraint.  Thus, if we can learn edges, then we can get the rows of $A$ and the entries of $\bbb$.   The major difference between what we did in the $m=d$ case is that now many edges may intersect one edge at multiple locations.  We show in two dimensions that this does not cause a problem.  
\ifnum\final=0
\subsubsection*{Algorithm}
\else
\subsubsection{Algorithm}
\fi

At each round, the observer will make a prediction $\hat\bbx^{(t)}$ based on the previous solutions he has seen, and if he is wrong, he will update his guess for the unknown constraints of the LP.  By Assumption \ref{assumpt:distinct}, if the known constraint binds i.e. $\bp\utt\cdot\bbx\utt= q\utt$, then with probability one $\bbx\utt$ will be distinct from previously seen points.  Furthermore, given Assumption \ref{assumpt:bind} and $d=2$, when the known constraint binds, there is exactly one constraint in the underlying LP that binds as well.  Using Lemma \ref{lem:edge}, we know that once we see three points that are collinear (using the procedure $\coline$) then all three points must bind the same constraint. Thus, we can combine these observations to learn the edge $\bbe$ where
\ifnum\final=0$
\else
$$
\fi
\bbe = \{\bbx\in \R^2 : A_i \bbx = b_i \text{ for some } i \in [m] \}.
\ifnum\final=0$
\else
$$
\fi
%Hence, $\bbe$ is exactly the line where the $i$th constraint in the LP binds and learning edges is the same as learning constraints.  

As we mentioned before, edges of the polytope in two dimensions correspond to the unknown constraints, however we do not learn which direction the inequality goes with each constraint.  Our algorithm then continues by learning rows of the matrix $A$ and entries in the right hand side vector $\bbb$ by learning edges.  Once we have seen a point that is not on the learned edge, then we would know the direction of the inequality for the learned constraint.  Further, once we learn other edges, we would also learn the direction of the inequality for the corresponding constraints.  

%The algorithm needs to learn the objective function as well. We show that when the algorithm makes a mistake and the the point we see is on one of the constraints of the LP that we have learned, then we can update our guess for the objective function by running the Ellipsoid Algorithm ($\ellip$).  

We formally outline the procedure described above in the procedure $\learntwo$ given in Algorithm~\ref{alg:2d} \ifnum\final=1 in the appendix\fi. In the $\learntwo$, we used the notation $LP\utt$ for $\left(A\utt,\bbb\utt\right)$.

\ifnum\final=1
ADD HIGH LEVEL HERE
\fi

\ifnum\final=0
\begin{algorithm}[h]
 \begin{algorithmic}
 \State Observer uses $\learntwo(\cA) = \learnedge(\cA,\cI^{(0)},\predtwo,\uptwo)$ against $\cA$, where:
 \State (\emph{Initialize})
\State $\quad \cI^{(0)} \gets \left\{LP^{(0)} = (A^{(0)}, \bbb^{(0)}) \gets ([],[]),  S^{(0)} \gets \emptyset.\right\}$
\\
 \Procedure{$\predtwo$}{$\cI = (\hat{LP},S),(\bp,q),\bbx^*$}
\If{$\bbx^* \neq \bot \quad \& \quad\bp\cdot\bbx^* < q$}
	$\hat \bbx \gets \bbx^*$
\ElsIf{$\hat{LP}$ has at least 1 row}
	\If{$\hat A, \hat b$ has one row and $\forall \bbz \in S$ it holds $\hat A \bbz = \hat\bbb$}
		\If{$\exists \hat \bbz \in \{\bbz: \hat A\bbz = \hat b \} \cap \{\bbz:  \bp\cdot \bbz = q\}$}
			$\hat \bbx \gets \hat\bbz$
		\Else   $\quad\hat \bbx \gets$ some arbitrary point
		\EndIf
	\Else
	\begin{align}
	\hat \bbx \gets \argmax_{x}\left\{\bbc \cdot \bbx:   \bp \cdot\bbx = q \quad \& \quad \hat A \bbx \leq \hat \bbb\right\}
	\label{eq:predtwo}
	\end{align}
	\EndIf
 \Else   $\quad\hat\bbx \gets$ some arbitrary point.
\EndIf
  \Return $\hat\bbx$ \Comment{Prediction}
\EndProcedure
\\
\Procedure{$\uptwo$}{$\cI = (\hat{LP},S),\bbx$}
 \If{$\coline( S , \bbx)$ produces two points $\bby^{1}, \bby^{2}$}
 	\State Let $\mathbf{a}$ be the normal to the line that includes $\bby^{1},\bby^{2}$ and $b$ be the intercept.
	\If{$\hat{LP} == ([],[]) \quad \& \quad \exists \bbz \in S$ such that $\mathbf{a}\cdot \bbz \neq b$}
		\If{$\mathbf{a}\cdot \bbz > b$}
			 $\mathbf{a} \gets -\mathbf{a}$ and $b \gets -b$.  \Comment{Flip inequality}
		\EndIf
	\ElsIf{$\hat A,\hat\bbb$ has at least one row}
		\If{$\exists \bbz \in S$ such that $\mathbf{a}\cdot\bbz > b$}
			 $\mathbf{a} \gets -\mathbf{a}$ and $b \gets -b$. 
		\EndIf
	\EndIf
	 
	\State $\hat A\leftarrow [\hat A;\mathbf{a}]$, $\hat\bbb\leftarrow[\hat\bbb;b]$. \Comment{Add row $\mathbf{a}$ to $\hat A$ and element $b$ to vector $\hat\bbb$}
% \ElsIf{$\exists j$ such that $\hat A_j \bbx = \hat b_j$}
 %	\State  $ H = \{\bbc \in \R^2 : \bbc \cdot \bbx \geq \hat\bbc \cdot \bbx \}$, $\cE \gets \ellip(H, \cE)$, $\hat\bbc \gets $ Center point of $\cE$.
 \EndIf
 \State $S \gets S \cup \{\bbx \}$ 
   \State\Return $\cI = (\hat{LP}, S)$ \Comment{Updates}
\EndProcedure
\end{algorithmic}
\caption{Two Dimension Procedure ($\learntwo$)}
\label{alg:2d}
\end{algorithm}
\fi

%Furthermore, we assume that 
%that $||\bbc||_2 \leq 1$ so it suffices to set $\cE^{(0)}$ as in Algorithm~\ref{alg:2d} to guarantee that the actual objective function $\bbc \in \R^2$ is included
%in the initial ellipsoid.

%\sj{Is the separating hyperplane correct?}
\ifnum\final=0
\subsubsection*{Analysis}
\else
\subsubsection{Analysis}
\fi

Similar to Section~\ref{sec:few-analysis}, we divide the mistakes that the $\predtwo$ can make into different categories. We start 
by mistakes of type zero given in \eqref{eq:mistake0}, i.e. when the new constraint does not bind.  
%Note that in this section we will not need to explicitly assume Assumption \ref{assumpt:bind} if we have Assumptions \ref{assumpt:rank} and \ref{assumpt:distinct} because with probability one the new constraint that is added each day will define a line that is linearly independent of each individual row of $A$.  


\begin{lemma}
\label{lem:mistake1}
The number of mistakes of type zero, defined in Equation~\eqref{eq:mistake0}, the observer can make when using procedure $\learntwo(\cA)$ given in Algorithm~\ref{alg:2d} is at most one, i.e.
\ifnum\final=0$
\else
$$
\fi
M_0 \leq 1.
\ifnum\final=0$
\else
$$
\fi
%\label{lem:type1}
\end{lemma}
\ifnum\final=0
\begin{proof}
The proof is exactly the same as the proof of Lemma \ref{lem:mistake1}.
\end{proof}
\fi

We then consider mistakes of the type when the additional constraint binds each day.  Note that we are no longer updating some edge set $E$, but rather we are creating a feasible region by learning the actual constraints of the underlying LP in \eqref{eq:LP}.  
\sj{type to be filled}

\begin{lemma}
We assume that Assumptions \ref{assumpt:rank} and \ref{assumpt:bind} hold.  For each round $t$, every row of $A\utt$ and $\bbb\utt$ in $\learntwo$ is a row of the unknown matrix $A$ and the unknown right hand side vector $\bbb$, respectively.
\label{lem:2d-constraints}
\end{lemma}
\ifnum\final=0
\begin{proof}
$\uptwo$ adds a row to $A\utt$ and $\bbb\utt$ after observing three collinear points that bind the added constraint on the days they were seen.  By Lemma \ref{lem:edge}, we know that these three points form an edge of the underlying polytope, so for $d=2$ only one row of the underlying matrix binds.  Thus, we learn $\bbe^i = \{\bbx \in \R^2: A_i\bbx = b_i \}$ for some $i \in [m]$ after seeing three collinear points.  
\end{proof}
\fi

Note that in $\predtwo$, once we have learned a constraint, there is the case when we may not know the direction of the inequality because we have only seen points that bind that constraint.  This can only occur when we only know a single constraint of the underlying LP and we have never seen a point that does not bind that constraint.  In that case, $\predtwo$ will only guess points that bind the added constraint and the learned constraint.  If we ever guess incorrectly, then the adversary must have shown a point that does not bind the constraint we have learned.  Further, once we know the direction of the inequality in the constraints, then we use \eqref{eq:predtwo} to find the best feasible point that we know so far.  Hence, every time we make a mistake, the adversary is showing a point that binds a constraint that is not learned yet.  

Let us consider mistakes of the following type
\begin{equation}
M^{2D}_1 = \sum_t \1\left\{\hat\bbx\utt \neq \bbx\utt : \bp\utt\cdot\bbx\utt = q\utt \right\}
\label{eq:mistake1_2d}
\end{equation}
\sj{why this is different than mistakes of type 1 in the previous section?}
We then have the following result.

\begin{lemma}
We assume that Assumptions \ref{assumpt:rank}, \ref{assumpt:bind}, and \ref{assumpt:distinct} hold.   If an observer uses $\learntwo(\cA)$ against $\cA$ then we have 
\ifnum\final=0$
\else
$$
\fi
M^{2D}_1 \leq 3m
\ifnum\final=0$
\else
$$
\fi
$\quad$ where $M^{2D}_1$ is given in \eqref{eq:mistake1_2d}
\label{lem:2d-m1}
\end{lemma}
\ifnum\final=0
\begin{proof}
We only consider the case that the added constraint each day binds.   It must then be the case that $\bbx\utt$ binds one of the rows of $A$ and  $\bbb$.  From Lemma \ref{lem:2d-constraints}, we know that each time we update via \eqref{eq:predtwo} then we only make a mistake if the point we predict violates an unknown constraint and the actual solution binds a constraint we have not learned.  Further, if we do not use \eqref{eq:predtwo} to predict $\hat\bbx\utt$, then we can only make a mistake if again we see a point that binds a constraint we have yet to learn.  

Thus, the only way we can make a mistake when the added constraint does not bind is if the actual point is binds a constraint that has not been learned yet.  By Assumption \ref{assumpt:distinct} and because we learn constraints after seeing three points that are collinear by Lemma \ref{lem:edge}, the lemma follows.  



By Assumption~\ref{assumpt:distinct}, each time $\bbx\utt$ is on an unknown constraint then it must be distinct from other points on that edge.  This can occur at most $3m$ times because there are $m$ rows of $A$ and we learn the rows after seeing three distinct points that bind the unknown constraint. 
\end{proof}
\fi
%
%We define another type of mistake: the number $M_3$ of mistakes of type three are the number of rounds that the $\bbx\utt$ is on the boundary of one of the constraints 
%discovered by $\uplp$ beforehand but $\predlp$ still predicts incorrectly, i.e.
%$$
%M_3 = \sum_t \1\left\{ \hat\bbx\utt \neq \bbx\utt :  \exists j \text{ s.t. }A\uttb_j \bbx\utt = b_j\uttb\right\}.
%$$
%
%We then consider mistakes of type two i.e., when the observer could have guessed correctly because the given point was on an edge that was known at that time, but he still guessed incorrectly.  
%
%\begin{lemma}
%Let $T_{EA}$ be the number of updates the Ellipsoid Algorithm needs to run in order to learn the objective function exactly.  Given Assumptions \ref{assumpt:rank}, \ref{assumpt:bind}, the number of mistakes of type one, defined in Equation~\ref{eq:mistake2}, made by Algorithm~\ref{alg:2d} is bounded by 
%$$
%M_2 \leq T_{EA}
%$$
%\label{lem:2d-m3}
%\end{lemma}
%\begin{proof}
%We show that whenever $\predtwo$ makes mistakes of type two, then the current guess for the objective function must be incorrect. This will prove that the number of mistakes of type two is bounded by the number of updates the Ellipsoid Algorithm needs to make in order to learn the objective function exactly.
%
%First observe that $\predtwo$ does not make any mistakes of type two when there are at most one learned  constraint by $\uptwo$.  So then we consider the case when at least two constraints are known at round $t$ and $\predtwo$ makes a mistake of type two.  
%
%We consider the prediction $\hat\bbx\utt$ and the constraint that it binds $A\uttb_i\hat\bbx\utt = \bbb\uttb_j$ along with the actual solution $\bbx\utt$ and the constraint that it binds $A\uttb_j\bbx\utt = \bbb\uttb_j$, where $i \neq j$.  We know $\bbc\uttb\cdot\bbx\utt \leq \bbc\uttb\cdot\hat\bbx\utt$. So either the estimate $\bbc\uttb$ is incorrect or there exists some unknown constraint that makes $\hat\bbx\utt$ infeasible, i.e. $A_\ell \hat\bbx\utt > b_\ell$ for $\ell \neq i$. 
%
%If we are in the first case, we can update the objective. We show that the second case cannot occur.  Consider the line segment connecting $\hat\bbx\utt$ and $\bbx\utt$. Starting from $\hat\bbx\utt$ consider the first 
%point, $\bbx$, where the line and the feasible region of the polytope intersect, i.e. $A_\ell\bbx=\bbb_\ell$. Since $\bbx\utt$ is feasible we know $A_\ell \bbx\utt \le b_\ell$.  Further, by Assumption \ref{assumpt:distinct} we know that $\bbx\utt$ binds exactly two constraints, namely constraint $j$ and the added constraint, so then $A_\ell \bbx\utt < b_\ell$ and thus $\bbx\utt \neq \bbx$ and $\hat\bbx\utt\neq \bbx$.
%
%
%Note that the objective is decreasing on the line segment from $\hat\bbx\utt$ to $\bbx\utt$ and this contradicts
%the assumption that $\bbx\utt$ is the optimal solution on day $t$. Since the algorithm has not learned the $\ell$th constraint, then the potential mistake in this case would not 
%be considered a type two mistake.
%\end{proof}

Putting all the pieces together, we bound the number of mistakes of $\predtwo$ in Theorem~\ref{thm:mistake_2d}. 
%with a finite precision bound assumption on the elements of the objective function.

\begin{theorem}
If Assumptions~\ref{assumpt:rank} and \ref{assumpt:distinct} hold, the procedure that has the observer make predictions based on $\predtwo$ and updates by $\uptwo$ can make a finite number of mistakes $M$, where
$\ifnum\final=0$\fi
M =O(m).
$\ifnum\final=0$\fi
\label{thm:mistake_2d}
\end{theorem}
\ifnum\final=0
\begin{proof}
The proof is immediate from Lemmas~\ref{lem:mistake1}~and~\ref{lem:2d-m1}.
%\sj{the same comment as in proof of Theorem~\ref{thm:m=d}.}
%\rynote{Should be ok now}
\end{proof}
\fi
%\remark{We do not need Assumption \ref{assumpt:bind} in Section~\ref{sec:2d}.}
%\rynote{This remark cannot be true because we need Lemma \ref{lem:edge} and in order for the hypotheses to hold we need Assumption \ref{assumpt:bind}}
%\subsubsection{Adding More Constraints}
%\label{sec:2d-more}
%So far in this section, we only considered the case that one constraint is added each day.  We now consider the case when we see $P\utt \in \R^{k\times 2}$ and $\bq\utt \in \R^{k\times 1}$ where $k \geq 1$.
%
%By Assumption~\ref{assumpt:bind}, the number of new constraints that can possibly bind on each day is two in two dimensions.  Hence, if the two new constraints bind on a given day, that must mean that the objective estimate in $\predlp$ is incorrect, hence, it can be updated in the next iteration by $\uplp$.  If none of the new constraints bind and $\predlp$ guesses incorrectly, we are in a mistake of type one, which we can bound by 1 as shown in Lemma \ref{lem:type1}.
%
%We are then left to consider the case when a single new constraint binds.   This is precisely the case that we considered above in mistakes of type two and three.  Thus, the observer can use the same procedure of predicting with $\predlp$ and updating with $\uplp$.  Therefore, Theorem \ref{thm:mistake_2d} still holds when the number of new constraints added each day is $k\geq 1$.  
